Physical insights on fractal analysis applied to light curves $\delta$ Scuti stars

Fractal fingerprints have been found recently in the light curves of several {\delta} Scuti stars observed by CoRoT satellite. This sole fact might pose a problem for the detection of pulsation frequencies using classical pre-whitening techniques, but it is also a potentially rich source for information about physical mechanisms associated to stellar variability. Assuming that a light curve is composed by a superposition of oscillation modes with a fractal background noise, in this work we applied the Coarse Graining Spectral Analysis (CGSA), an FFT based algorithm, which can discriminate in a time series the stochastic fractal power spectra from the harmonic one. We have found that the fractal background component is determining the frequency content extracted using classical pre-whitening techniques in the light curves of {\delta} Scuti stars. This might be crucial to understand the amount of frequencies excited in these kind of pulsating stars. Additionally, CGSA resulted to be relevant in order to extract the oscillation modes, this points to a new criterion to stop the pre-whitening cascade based on the percentage of fractal component in the residuals.

==> Tables/table_CGSA_6Stars.tex <==
\begin{table*}
	\caption{Coarse Grained Spectral Analysis $\%Frac$ for the 6 CoRoT \dss ($7:37\cdot10^5$ points and 32 seconds of time step) under study. Here one could compare the $\%Frac$ value obtained with the whole light curve, the ones obtained with $\simeq 22$ days long curves ($L=6\cdot 10^4$), and the ones resulting from the harmonics sum model (HSM).}
    
    \label{tab:CGSA_6Stars}
	\begin{tabular}[!h]{lcccc}
ID $\delta$-Scuti & $\%Frac$ (Total length) & $\%Frac$  & $\%Frac$ HSM  & $\%Frac$ HSM PhRnd\\
\hline
HD174936 & 0.1161 & $0.133$ & $0.077$ & $0.098\pm0.030$\\ 
HD174966 & 0.0082 & $0.011$ & $0.006$ & $0.011\pm0.003$\\ 
HD48784 & 0.2779 & $0.256$ & $0.437$ & $0.426\pm0.058$\\ 
HD49434 & 0.2697 & $0.458\pm0.071$ & $0.668\pm0.055$ & $0.618\pm0.064$\\ 
HD50844 & 0.0567 & $0.084\pm 0.005$ & $0.138\pm0.009$ & $0.136\pm0.10$\\ 
HD50870 & 0.0191 & $0.036\pm 0.003$ & $0.058\pm0.010$ & $0.087\pm0.034$
\end{tabular}
\end{table*}

==> Tables/table_CGSA_fBm.tex <==
\begin{table*}
	\caption{Mean and standard deviation from the distributions obtained by $330$ fBm runs of $L=36409$ long time series, with Hurst exponent $\alpha$.}
    \label{tab:CGSA_fBm}
	\begin{tabular}[!h]{ccc}
$\alpha$ & $\mu(\%Frac)$ & $\sigma(\%Frac)$  \\
\hline
$1.125$  & $1.06$ & $0.17$ \\ 
$1.5$  & $1.03$ & $0.33$ \\
$1.875$  & $1.01$ & $0.31$ \\
\hline
	\end{tabular}
\end{table*}



==> Tables/table_CGSA_fGn.tex <==
\begin{table*}
	\caption{Mean and standard deviation from the distributions obtained by $330$ fGn runs of $L=36409$ long time series, with Hurst exponent $\alpha$. }
    \label{tab:CGSA_fGn}
	\begin{tabular}[!h]{ccc}
$\alpha$ & $\mu(\%Frac)$ & $\sigma(\%Frac)$  \\
\hline
$0.125$  & $1.01$ & $0.01$ \\ 
$0.5$  & $1.11$ & $0.01$ \\
$0.875$  & $1.07$ & $0.04$ \\
\hline
	\end{tabular}
\end{table*}

==> Tables/table_Oct.tex <==
\begin{table*}
	\caption{Rescaled Range exponent $\alpha$, Multifractal exponent $\alpha$ and Multifractal Singularity Spectra amplitude $\Delta\bar{\alpha}$ for CoRoT \dss ($7:37\cdot10^5$ points and 32 seconds of time step) under study. The broadness of Multifractal Singularity Spectra is thin \textbf{[compared with solar-like curves (data not shown)]CHECK}, and the only curve that seems to have a multifractal behaviour is the HD48784 \textbf{NO SE SI DEJAR LA COLUMNA DEL MULTIFRACTAL SPECTRA WIDTH, A LO MEYOR LO QUITARIA PARA OTRA PUBLICACION MAS ROBUSTA SOBRE MSS APLICADO A TODAS LAS 15 DSCUTI} }
    \label{tab:Oct}
	\begin{tabular}[!h]{lccc}
ID $\delta$-Scuti & RR $\alpha$ & MSS $\alpha$ & $\Delta\bar{\alpha}$ \\
\hline
GSC00144-03031 & 0.14 & & \\
HD170699 & 0.32 & & \\
HD172189 & 0.24 & & \\
HD174532 & 0.25 & & \\
HD174589 & 0.21 & & \\
HD174936 & 0.41 & 0.52 & 0.46 \\ 
HD174966 & 0.16 & 0.18 & 0.26 \\ 
HD181555 & 0.31 & & \\
HD41641 & 0.34 & & \\
HD48784  & 0.52 & 0.48 & 1.18 \\
HD49434  & 0.67 & 0.47 & 0.15 \\
HD50844  & 0.24 & 0.23 & 0.27 \\ 
HD50870  & 0.31 & 0.37 & 0.38 \\
HD51359  & 0.35 & & \\
HD51722  & 0.26 & & 
\end{tabular}
\end{table*}

%se devo aggiungere il CGSA
% HD174936 & 0.1161 \\ 
% HD174966 & 0.0082 \\ 
% HD48784 & 0.2779 \\ 
% HD49434 & 0.2697 \\ 
% HD50844 & 0.0567 \\ 
% HD50870 & 0.0191 

==> Tables/table_Stars.tex <==
% \begin{table*}
% 	\caption{Physical properties of the 6 CoRoT \dss ($7:37\cdot10^5$ points and 32 seconds of time step) under study. \textbf{Antonio va a trabajar esta tabla, anhadiendo o quitando parametros}}    
% \label{tab:Stars}
% 	\begin{tabular}[!h]{lccccccc}
% ID $\delta$-Scuti & $\Delta\nu(\mu Hz)$ & FT $\nu_{max}(\mu Hz)$ & Teff &	log(g) & $v\cdot sin(i)$ & SpT & Obs. Time (days) \\
% \hline
% HD174936 & 50 &	14,42 &	8000(200) &	4.08(0.2) &	169.7 &	A2 & 27.194 \\
% HD174966 & 63 & 34 & 7555(50) &	4.21(0.05) & 126.1(1.2) & A3 & 27.197 \\
% HD48784 & 54 & 14,73 & 6918.31 &           &108 & F0 & 25.305 \\ 
% HD49434 & 23 & 11,41 & 7244.36 &		   &     &F1 V&	136.89 \\
% HD50844	& 24 & 24,017 & 7400(200) & 3.6(0.2) & 58(2) & A2 &57.713 \\
% HD50870	& 28 & 93,15 & 7660(250) & 3.68(0.25) &	37.5(2.5) &	A8 III & 114.413
% \end{tabular}
% \end{table*}

\begin{table*}
	\caption{Physical properties of the 6 CoRoT \dss\ ($7:37\cdot10^5$ points and 32 seconds of time step) under study. Uncertainties, when available, are indicated in parenthesis.} \label{tab:Stars}
	\begin{tabular}[!h]{lccccccc}
ID $\delta$-Scuti & $\Delta\nu\ (\mu Hz)$ & FT $\nu_{max}\ (\mu Hz)$ & Teff (K) & log(g) & $v\cdot sin(i)$ (km$\cdot$s$^{-1}$) & SpT & Obs. Time (days) \\
\hline
HD174936 & 50 &	14,42 &	8000(200) &	4.08(0.2) &	169.7 &	A2 & 27.194 \\
HD174966 & 63 & 34 & 7555(50) &	4.21(0.05) & 126.1(1.2) & A3 & 27.197 \\
HD48784 & 54 & 14,73 & 6990(140) &           &108 & F0 & 25.305 \\ 
HD49434 & 23 & 11,41 & 7503(255) &	4.43(0.2)  &  85.7(4.3) & F1 V &	136.89 \\
HD50844	& 24 & 24,017 & 7400(200) & 3.6(0.2) & 58(2) & A2 &57.713 \\
HD50870	& 28 & 93,15 & 7660(250) & 3.68(0.25) &	37.5(2.5) &	A8 III & 114.413
\end{tabular}
\end{table*}

==> Tables/table_technicals.tex <==
\begin{table*}
	\caption{Temporal ranges, measured in days, considered for the calculation of MSS with the wavelet WTMM method. For the WTMM method the $\kappa$ parameters involved in the peaks correction window size (equation \ref{k_correction} is specified.}
    \label{tab:technical}
	\begin{tabular}[!h]{lc}
ID $\delta$-Scuti & MSS WTMM range ($\kappa$)\\
\hline
HD174936 & $0.117:1.171$  ($1.5$) \\ 
HD174966 & $0.370:3.704$  ($5.0$)\\
HD48784  & $1.171:11.712$ none \\
HD49434  & $3.704:37.037$ ($1.0$) \\
HD50844  & $0.370:11.712$ ($1.0$) \\
HD50870  & $0.370:6.586$  ($2.5$) \\ 
	\end{tabular}
\end{table*}
